Still not there? Comparing Traditional Sequence-to-Sequence Models to Encoder-Decoder Neural Networks on Monotone String Translation Tasks

We analyze the performance of encoder-decoder neural models and compare them with well-known established methods. The latter represent different classes of traditional approaches that are applied to the monotone sequence-to-sequence tasks OCR post-correction, spelling correction, grapheme-to-phoneme conversion, and lemmatization. Such tasks are of practical relevance for various higher-level research fields including digital humanities, automatic text correction, and speech recognition. We investigate how well generic deep-learning approaches adapt to these tasks, and how they perform in comparison with established and more specialized methods, including our own adaptation of pruned CRFs.

==> related.tex <==
\section{Related Work}
\label{sect:related}

\newcite{springmann_ocr_2014} give a detailed overview of the problems and challenges in the field of OCR post-correction.
In previous works, the noisy-channel model has been adopted for error correction by \newcite{brill_improved_2000}. The model has been improved by integrating phonetic information \cite{toutanova_pronunciation_2002} and by repetitive application in order to discover more complex errors \cite{cucerzan_spelling_2004}. \newcite{gubanov_improved_2014} further improved this approach with stochastic iterative correction.

Like in the noisy-channel approach \cite{brill_improved_2000}, \newcite{xu_probabilistic_2014} perform complex substring-to-substring substitutions with an efficient log-linear model, suitable for correcting spelling mistakes and other string-to-string translation tasks. \newcite{okazaki_discriminative_2008} suggest a general discriminative model for string-to-string translation.


\newcite{reffle_unsupervised_2013} present the interactive tool PoCoTo in which users manually mark errors. 
\cite{farra_generalized_2014} propose a generic character-based error identification and correction model, tested on Arabic data. 

Neural networks have been explored for spelling corrections earlier \cite{lewellen_neural_1998,raaijmakers_deep_2013}.
For the broader tasks of text normalization, grammar correction, and error identification, recurrent neural networks \cite{chrupala_normalizing_2014} and encoder-decoder models have been applied in recent works \cite{xie_neural_2016,schmaltz_sentence-level_2016}.


For the grapheme-to-phoneme conversion task, the methods implemented in our baseline systems also reflect the most important related work \cite{jiampojamarn_integrating_2010,jiampojamarn_joint_2008,novak_wfst-based_2012,bisani_joint-sequence_2008}, described in Section~\ref{sect:baseline}.


==> table_times.tex <==


\begin{center}
\begin{tabular}{| l | c | c | c | c | }
\hline
\textbf{Training Time in Sec.} & \textbf{Combilex (20K)} & \textbf{Combilex (10K)} & \textbf{Combilex (5K)} & \textbf{Combilex (2K)} \\
\hline
attn-enc-dec (1-100) & 5.3K & 3K & 1.8K	& 0.6K \\ 
attn-enc-dec (1-200) & 20.5K & 10K & 5.8K & 2.5K \\ 
attn-enc-dec (2-100) & 10.8K & 6.2K & 2.7K & 1.3K \\ 
attn-enc-dec (2-200) & 65.4K & 39K & 23.1K & 11.1K \\
attn-enc-dec (2-300) & & & & \\ 
attn-enc-dec (3-200) & 84.4K & 51.7K & 25.3K & 19.4K \\ 
\hline
enc-dec (1-100) & 5.1K & 2.9K & 1.7K & 0.7K \\ 
enc-dec (1-200) & 18.9K & 9.8K & 5.2K & 2.3K \\ 
enc-dec (2-100) & 11.3K & 5.8K & 3.4K & 1.7K \\ 
enc-dec (2-200) & 75.8K & 40.2K & 16.4K & 11.3K \\ 
\hline
morph-trans (1-100) & 5K & 2.4K & 1.1K & 0.5K \\ 
morph-trans (1-200) & 26.9K & 13.9K & 6.4K & 3.2K \\ 
morph-trans (2-100) & 9.4K & 5.1K & 2.6K & 0.9K \\ 
morph-trans (2-200) & 72.9K & 43.7K & 20K & 8.9K \\ 
\hline
PCRF (order 1) & & & & \\
PCRF (order 3) & & & & \\ 
PCRF (order 4) & & & & \\ 
PCRF (order 5) & & & & \\ 
\hline DirectTL+  & & & & \\ 
\hline Phonetisaurus ($n=8$) & \textbf{46} & \textbf{26} & \textbf{14} & \textbf{6} \\ 
\hline Sequitur  & 4K & 1.6K & 0.8K & 0.2K \\ 
\hline 
\end{tabular}
\end{center}
\caption{Training time in seconds for all systems on the Combilex training sets of different sizes.} 

